ThermoSight: From Appearance to Internal Thermofluid Fields via Physics-Guided Neural Reconstruction

Most neural reconstruction methods focus on reproducing scene appearance, yet inferring physical states from visual observations is essential for machine understanding of the physical world. Reconstructing the internal temperature and soot fields of radiating thermofluids such as flames is challenging yet essential for improving energy efficiency and assessing heat exposure and fire spread. In flames, temperature and soot concentration jointly govern visible emission, and soot self-absorption alters the light that reaches each camera. With limited views, changes in the two fields can offset one another in the recorded RGB images, making temperature and soot difficult to disentangle. ThermoSight, a physics-guided neural framework for scientific imaging, jointly reconstructs continuous three-dimensional temperature and soot volume fraction fields from limited calibrated flame images without field-level ground truth during optimization. A differentiable spectral model links these fields to measured RGB through thermal emission, self-absorption, and calibrated camera responses. Temperature-dependent emission spectra and wavelength-dependent attenuation constrain shared fields across RGB channels, reducing temperature-soot ambiguity. Chromaticity consistency, observation-derived spatial constraints, and soot regularization complement intensity fitting. In a synthetic ablation, wavelength-resolved attenuation reduces temperature RMSE in the hot, sooty region from 234 to 112 K relative to a three-channel approximation, with nearly identical RGB PSNR (65.23 vs. 65.24 dB). Measured data yield coherent fields and competitive RGB reconstructions. These results demonstrate that physics-guided neural fields recover interpretable internal physical quantities beyond visually consistent appearance.

==> sec/supp_contents.tex <==
\makeatletter
\begingroup
\setcounter{tocdepth}{2}
\newcommand{\suppcontentsentry}[2]{%
  \csname l@#1\endcsname{%
    \hyperref[#2]{\numberline{\ref*{#2}.}{\let\texorpdfstring\@secondoftwo\nameref*{#2}}}%
  }{\pageref*{#2}}%
}
\suppcontentsentry{section}{sec:supp_additional_conditions}
\suppcontentsentry{section}{sec:supp_acquisition_and_implementation}
\suppcontentsentry{subsection}{sec:supp_acquisition}
\suppcontentsentry{subsection}{sec:supp_implementation}
\suppcontentsentry{subsection}{sec:supp_spectral_derivations}
\suppcontentsentry{section}{sec:supp_convergence}
\suppcontentsentry{section}{sec:supp_mismatch}
\endgroup
\makeatother

